Socket Intents: OS Support for Using Multiple Access Networks and its Benefits for Web Browsing

In today's Internet, mobile devices are connected to multiple access networks, e.g., WiFi/DSL and LTE. To take advantage of the networks' diverse paths characteristics (delay, bandwidth, and reliability) and aggregate bandwidth, we need smart strategies for choosing which interface(s) to use for what traffic. In this paper, we present an approach how to tackle this challenge as part of the Operating System (OS): With the concept of Socket Intents, applications can express what they know about their communication pattern and their preferences. Using our Socket Intents Prototype and our modified BSD Socket Interface, this information is used to choose the most appropriate path or path combination on a per message or per connection basis. We evaluate our system based on the use case of Web browsing: Using our prototype and a client-side proxy, we show the feasibility and benefits of our design. Using a flow-based simulator and a full factorial experimental design, we study a broad range of access network combinations (based on typical DSL and LTE scenarios) and real workloads (Alexa Top 100 and Top 1000 Web Sites). Our policies achieve performance benefits in more than 50% of the cases and speedups of more than factor two in 20% of the cases without adding overhead in the other cases.

==> policies.tex <==
\section{Socket Intents Policies}
\label{sec:policies}

\todo[inline]{This section has passed away … its remains remain here for the only purpose of being copied over to the evaluation or being deleted … not a shame as the content lives on}

In this paper, we present the \eafpolicy as it fits our use case of Web
browsing: Objects of different sizes can be fetched over different interfaces
and the download time largely depends on the object's file size as well as the RTT and
available bandwidth on the path. We use the \filesizeIntent, which allows an
application, e.g. an HTTP client, to communicate the size of each object as a
communication unit which is to be transferred. The policy then chooses the
more suitable interface for it. Assuming that there are at least two access
networks and they vary in RTT and bandwidth, our intuition is that if the
communication unit is small, the policy should choose the interface with the
shorter RTT. If the communication unit is large it should prefer the interface
with the larger available bandwidth. Thus, each unit is scheduled on the interface
with the earlier arrival time, resulting in a shorter overall completion time.

We compare this policy against several baseline cases including vanilla MPTCP. 
We also combine this policy with MPTCP to distribute an object download over both
interfaces.


\subsection{Policy Description}

\begin{description}

\item[{Single Interface}]
This policy always chooses a particular, statically configured interface.

\item[{Round Robin}]
This policy uses multiple interfaces on a round robin basis.

\item[{Earliest Arrival First (EAF)}]
This policy uses the \filesizeIntent to predict the completion time for each
available interface. It then chooses the one where the communication unit
will arrive first. The prediction is based on an estimation of the interface
RTT and available bandwidth. 

\item[{MPTCP}] 
This policy uses MPTCP with the full-mesh path manager across all interfaces. It presumes that MPTCP subflows can be opened on all local and remote interfaces. With two network interfaces at the client and one interface at the server,
the policy establishes two subflows. The interface for the initial subflow is configurable.
This policy considers neither the \socketintents nor the current network performance.

\item[{Earliest Arrival First with MPTCP (EAF\_MPTCP)}]
This policy combines the \poln{EAF} Policy with MPTCP.  In addition to predicting the
arrival time for each interface, it also considers MPTCP for all possible
interface combinations. The intuition here is that MPTCP is beneficial for
some cases but not all cases. For example, this policy can avoid scheduling
small communication units on a high RTT interface.  We expect that this policy
should give the best results.

\end{description}


\subsection{Policies Realization}
\label{sub:policies_eval}

To evaluate the benefits of our policies for Web traffic we realize them in our
Web transfer simulator as well as in our \prototype. The implementations of
\poln{Single Interface} and \poln{Round Robin} do not differ in behavior.

For \poln{EAF} the \prototype uses estimates of the minimum SRTT per prefix
and the available bandwidth as well as the maximum observed bandwidth per
interface. The object size for the \filesizeIntent is determined via a
two-step download that is described in detail in \sref{sec:proxy}.
\poln{EAF} estimates the available bandwidth as the difference
between the currently used bandwidth and the maximum observed bandwidth.  If since the
most recent measurement one or more downloads have been scheduled on an interface,
we reduce the available bandwidth in our calculation. Finally, we divide the file size by the
estimated available bandwidth to approximate the download duration.  We add one
RTT if a connection can be reused and two RTTs if a new connection has to
be established.  Finally, the interface with the shortest predicted arrival
time is chosen.  We do not consider TLS handshakes.

Since the simulator tries to provide an upper bound of the benefits it 
relies on its global knowledge  about all currently active transfers. 
The RTT and maximum interface bandwidth, as well as the size of the objects
for the \filesizeIntent, are known a priori. Thus, the policy predicts the 
arrival time of each communication unit by ``scheduling'' it on
each candidate interface and computing the download time. Finally, the policy
selects the interface with the earliest predicted arrival time.
Within the simulation, we add one RTT if a connection can
be reused, two RTTs if a new connection has to be established, and
two additional RTT for each TLS handshake.

For \poln{MPTCP}, we considered two variants: starting the initial MPTCP subflow on
the same statically chosen interface or always on a different, randomly chosen interface. The simulation of \poln{EAF\_MPTCP} is analogous to the EAF policy, but it includes
predictions with MPTCP for all interface combinations, therefore using the interface for
the first subflow that is predicted to give the best results. \footnote{We did not
implement MPTCP policies in the prototype as this promised no further insights.}



